Ranks of Tensor Networks for Eigenspace Projections and the Curse of Dimensionality

The hierarchical (multi-linear) rank of an order-$d$ tensor is key in determining the cost of representing a tensor as a (tree) Tensor Network (TN). In general, it is known that, for a fixed accuracy, a tensor with random entries cannot be expected to be efficiently approximable without the curse of dimensionality, i.e., a complexity growing exponentially with $d$. In this work, we show that the ground state projection (GSP) of a class of unbounded Hamiltonians can be approximately represented as an operator of low effective dimensionality that is independent of the (high) dimension $d$ of the GSP. This allows to approximate the GSP without the curse of dimensionality.

==> pratenddefaultcategory.tex <==

\label{proofsection:prAtEndii}\begin{proof}[Proof of \autoref{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}The operator $U(t):=\exp {\i Ht}\exp {-\frac {t^2}{2q}}$ is strongly continuous for all $t\in \R $. Thus, a finite integral of $U(t)$ is well defined. For any $\uu \in \X $ \begin {align*} \lim _{c\rightarrow \infty }\norm {\frac {1}{\sqrt {2\pi q}} \int _{-c}^cU(t)\uu \d t}[\X ]\leq \lim _{c\rightarrow \infty }\norm {\uu }[\X ]\frac {1}{\sqrt {2\pi q}} \int _{-c}^c\exp {-\frac {t^2}{2q}}\d t=\norm {\uu }[\X ]. \end {align*} Thus, the integral \eqref {eq:pq} is well defined. \par Since $H$ is self-adjoint, we have the spectral decomposition \begin {align*} H=\int _{\sigma (H)}\lambda \d P(\lambda ), \end {align*} where $P:\sigma (H)\rightarrow \LL {\X }$ is a projection valued measure. Due to the gap assumption, we get that $NP_0=P(\lambda _0)$. \par Applying functional calculus for self-adjoint operators \begin {align*} \exp {\i Ht}=\int _{\sigma (H)}\exp {\i \lambda t}\d P(\lambda ). \end {align*} Equation \eqref {eq:pq} is to be interpreted as the unique operator such that for any $\uu \in \X $ \begin {align*} \inp {\uu }{\frac {1}{\sqrt {2\pi q}}\int _{-\infty }^\infty U(t)\uu \d t}_{\X } &= \frac {1}{\sqrt {2\pi q}}\int _{-\infty }^\infty \exp {-\frac {t^2}{2q}}\inp {\uu }{U(t)\uu }_{\X }\d t\\ &= \frac {1}{\sqrt {2\pi q}}\int _{-\infty }^\infty \exp {-\frac {t^2}{2q}}\int _{\sigma (H)}\exp {\i \lambda t}\d P_{\uu }(\lambda )\d t, \end {align*} where $P_{\uu }(\cdot )=\inp {\uu }{P(\cdot )\uu }_{\X }$ and the equality follows from the linearity and continuity of the $\X $-inner product. For the last integral we can apply Fubini's Theorem for general product measures. This allows us to write \begin {align*} \rho ^q&=\frac {1}{N\sqrt {2\pi q}}\int _{-\infty }^\infty \int _{\sigma (H)} \exp {\i \lambda t}\exp {-\frac {t^2}{2q}}\d P(\lambda )\d t\\ &\overset {\text {gap}}{=}\frac {1}{N\sqrt {2\pi q}}\int _{-\infty }^\infty P_0\exp {-\frac {t^2}{2q}}+\int _{\sigma (H)\setminus \set {\lambda _0}} \exp {i\lambda t}\exp {-\frac {t^2}{2q}}\d P(\lambda )\d t\\ &\overset {\text {Fubini}}{=} P_0+\frac {1}{N\sqrt {2\pi q}}\int _{\sigma (H)\setminus \set {\lambda _0}} \int _{-\infty }^\infty \exp {\i \lambda t}\exp {-\frac {t^2}{2q}}\d t\d P(\lambda ). \end {align*} The last term is the Fourier transform of the density of the normal distribution. Thus, \begin {align*} \norm {\rho ^q-P_0}[\Lnorm ]=\frac {1}{N} \norm {\int _{\sigma (H)\setminus \set {\lambda _0}} \exp {-\frac {1}{2}\lambda ^2 q}\d P(\lambda )}[\Lnorm ] \leq \frac {1}{N}\exp {-\frac {1}{2}(\Delta E)^2q}, \end {align*} which completes the proof.\end{proof}
\label{proofsection:prAtEndiii}\begin{proof}[Proof of \autoref{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}By the same arguments as in Lemma \ref {lemma:pq}, the integrals are well defined. Next, application to the ground state yields \begin {align*} H_L(t)\uu _0&=\exp {\i Ht}H_L\int _{\sigma (H)}\exp {-\i \lambda t}\d P(\lambda ) \uu _0\overset {\lambda _0=0}{=}\exp {\i Ht}H_L\uu _0 = \int _{\sigma (H)}\exp {\i \lambda t}\d P(\lambda )H_L\uu _0\\ &=\inp {\uu _0}{H_L\uu _0}_{\H }\uu _0+\int _{\sigma (H)\setminus \set {\lambda _0}} \exp {\i \lambda t}\d P(\lambda )H_L\uu _0. \end {align*} Thus, \begin {align*} \tilde {H}_L\uu _0&=\frac {1}{\sqrt {2\pi q}}\int _{-\infty }^\infty H_L(t)\uu _0\exp {-\frac {t^2}{2q}}\d t\\ &=\int _{\sigma (H)\setminus \set {\lambda _0}}\frac {1}{\sqrt {2\pi q}} \int _{-\infty }^\infty \exp {\i \lambda t}\exp {-\frac {t^2}{2q}}\d t\d P(\lambda ) H_L\uu _0\\ &= \int _{\sigma (H)\setminus \set {\lambda _0}}\exp {-\frac {1}{2}\lambda ^2 q} \d P(\lambda )H_L\uu _0. \end {align*} On the other hand, \begin {align*} H\tilde {H}_L\uu _0=\int _{\sigma (H)\setminus \set {\lambda _0}} \lambda \exp {-\frac {1}{2}\lambda ^2q}\d P(\lambda )H_L\uu _0. \end {align*} Hence, \begin {align}\label {eq:hhl} \norm {H\tilde {H}_L\uu _0}[\X ]\geq \Delta E\norm { \int _{\sigma (H)\setminus \set {\lambda _0}}\exp {-\frac {1}{2}\lambda ^2q} \d P(\lambda )H_L\uu _0}[\X ]=\Delta E\norm {\tilde {H}_L\uu _0}[\X ]. \end {align} Next, since $H\uu _0=0$, \begin {alignat*}{2} H\tilde {H}_L\uu _0&=&&(H\tilde {H}_L-\tilde {H}_LH)\uu _0 =\int _{\sigma (H)\setminus \set {\lambda _0}}\exp {-\frac {1}{2}\lambda ^2q} \d P(\lambda )\comm {H}{H_L}\uu _0\\ &=&&\int _{\sigma (H)\setminus \set {\lambda _0}}\exp {-\frac {1}{2}\lambda ^2q} \d P(\lambda )\comm {H_{j-l-1,j-l}}{H_{j-l-2,j-l-1}}\uu _0\\ &=&&\int _{\sigma (H)\setminus \set {\lambda _0}}\exp {-\frac {1}{2}\lambda ^2q} \d P(\lambda ) \bigg \{ \comm {H_{j-l-1}}{(\Phi _{j-l-2,j-l-1}-\Phi _{j-l-1,j-l})}\\ & &&+\comm {\Phi _{j-l-1,j-l}}{\Phi _{j-l-2,j-l-1}}\bigg \}\uu _0, \end {alignat*} where the last equality follows from Assumption \eqref {ass:int}. And thus \begin {align*} \norm {H\tilde {H}_L\uu _0}[\X ]\leq 3J^2\exp {-\frac {1}{2}(\Delta E)^2q}. \end {align*} Together with \eqref {eq:hhl} \begin {align*} \norm {\tilde {H}_L\uu _0}[\X ]\leq 3J^2(\Delta E)^{-1}\exp {-\frac {1}{2}(\Delta E)^2q}, \end {align*} and analogously for $\tilde {H}_B$, $\tilde {H}_R$. This completes the proof.\end{proof}
\label{proofsection:prAtEndiv}\begin{proof}[Proof of \autoref{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}First, note that we can differentiate $H_L(t)$ to obtain \begin {align*} \frac {\d }{\d t}H_L(t)&=\frac {\d }{\d t}\exp {\i Ht}H_L\exp {-\i Ht}\\ &=\exp {\i Ht}\i HH_L\exp {-\i Ht}-\exp {\i Ht}iH_LH\exp {-\i Ht}\\ &=\exp {\i Ht}\i \comm {H}{H_L}\exp {-\i Ht} =:\i \comm {H}{H_L}(t), \end {align*} and $H_L(0)=H_L$. Thus, we can write \begin {align}\label {eq:thanks1} H_L(t)=H_L+\int _{0}^t\i \comm {H}{H_L}(\tau )\d \tau . \end {align} By Assumption, $\comm {H}{H_L}$ is bounded and supported on $\X _{j-l-2,j-l}$. Consequently, we can write \begin {align*} \tilde {H}_L=H_L+\frac {1}{\sqrt {2\pi q}}\int _{-\infty }^\infty \int _0^t\i \comm {H}{H_L}(\tau )\d \tau \exp {-\frac {t^2}{2q}}\d t. \end {align*} Since the commutator is bounded and local, and the interactions in $H$ are bounded, by \cite [Corollary 2.2]{LBInfDim}, we know a Lieb-Robinson bound applies to $\comm {H}{H_L}$. I.e., there exists a constant (velocity) $v\geq 0$ and constants $C>0$, $a>0$, such that \begin {align}\label {eq:lrbnd} &\norm {\comm {\comm {H}{H_L}(\tau )}{B}}[\Lnorm ] \leq C\norm {\comm {H}{H_L}}[\Lnorm ] \norm {B}[\Lnorm ]\exp {-a\left \{\dist (\comm {H}{H_L}, B)-v|\tau | \right \}}, \end {align} for all bounded and local $B$. Thus, by \cite [Lemma 3.2]{NearComm}, there exists a map $\Pi :\LL {\X }\rightarrow \LL {\X }$ such that $\Pi (A)$ is supported on $\X _{j-2l-2,j}$ and, for any $A\in \LL {\X }$ satisfying \eqref {eq:lrbnd} with $\dist (A, B)\geq l$, we have \begin {align*} \norm {A-\Pi (A)}[\Lnorm ]\leq 2C\norm {A}[\Lnorm ] \exp {-a\left \{l-v|\tau | \right \}}. \end {align*} Then, using \cite [Theorem 3.4]{NearComm}, we integrate over time and further estimate \begin {align*} &\norm {\int _{0}^t\comm {H}{H_L}(\tau )\d \tau - \int _0^t\Pi \left (\comm {H}{H_L}(\tau )\right ) \d \tau }[\Lnorm ] \leq |t|CJ^2\exp {-a\{l-v|t|\}}. \end {align*} \par We define the operator \begin {align*} \diff _L:=\frac {1}{\sqrt {2}\pi q}\int _{-\infty }^\infty \int _0^t \Pi \left (\i \comm {H}{H_L}(\tau )\right )\d \tau \exp {-\frac {t^2}{2q}} \d t. \end {align*} By all of the above, this operator is bounded and supported on $\X _{j-2l-2, j}$. Analogously, we define $\diff _B$ and $\diff _R$ with supports in $\X _{j-2l-2,j+2l+3}$ and $\X _{j+1, j+2l+3}$, respectively. \par What remains is to truncate the tails of the integral to obtain an overall error of the same order as the Lieb-Robinson bound. Let $T=\frac {l}{2v}$. Then, \begin {align}\label {eq:trunc} &\norm {\tilde {H}_L^1-M_L}[\Lnorm ]=\notag \\ &= \norm {\frac {1}{\sqrt {2\pi q}}\int _{-\infty }^\infty \int _{0}^t \left (\i \comm {H}{H_L}(\tau )- \Pi \left (\i \comm {H}{H_L}(\tau )\right )\right )\d \tau \exp {-\frac {t^2}{2q}}\d t}[\Lnorm ]\notag \\ &=\norm {\frac {1}{\sqrt {2\pi q}}\left ( \int _{|t|\leq T}\ldots +\int _{|t|>T}\ldots \right )}[\Lnorm ]\notag \\ &\leq CJ^2\exp {-al} \left (\exp {avT}\frac {1}{\sqrt {2\pi q}}\int _{|t|\leq T} |t|\exp {-\frac {t^2}{2q}}\d t+\frac {1}{\sqrt {2\pi q}}\int _{|t|>T} |t|\exp {av|t|-\frac {t^2}{2q}}\d t\right ). \end {align} For the first term \begin {align*} \frac {1}{\sqrt {2\pi q}}\int _{|t|\leq T} |t|\exp {-\frac {t^2}{2q}}\d t\leq \sqrt {\frac {q}{2\pi }}. \end {align*} For the second \begin {alignat*}{2} \frac {1}{\sqrt {2\pi q}}\int _{|t|>T} |t|\exp {av|t|-\frac {t^2}{2q}}\d t &=&&\sqrt {\frac {2}{\pi q}}\int _{T}^\infty t\exp {avt-\frac {t^2}{2q}}\d t\\ &=&&q\exp {avT-\frac {T^2}{2q}}\\ & &&+avq \int _T^\infty \exp {avt-\frac {t^2}{2q}}\d t. \end {alignat*} For the latter term \begin {align*} \int _T^\infty \exp {avt-\frac {t^2}{2q}}\d t&= \int _T^\infty \exp {\frac {(av)^2q}{2}- \left (\sqrt {\frac {1}{2q}}t-av\sqrt {\frac {q}{2}}\right )^2}\d t\\ &= \sqrt {2q}\int _{\sqrt {\frac {1}{2q}}T-av\sqrt {\frac {q}{2}}}^\infty \exp {-\tau ^2}\d \tau \leq \sqrt {\frac {q\pi }{2}}\exp {avT-\frac {T^2}{2q}}. \end {align*} And thus \begin {alignat*}{2} \norm {\tilde {H}_L-M_L}[\Lnorm ] &\leq && CJ^2\exp {-al}\times \\ & &&\bigg ( \exp {al/2}\sqrt {\frac {q}{2\pi }} +q\exp {al/2}\exp {-\frac {T^2}{2q}} +avq^{3/2}\sqrt {\frac {\pi }{2}}\exp {al/2}\exp {-\frac {T^2}{2q}} \bigg )\\ &\leq && CJ^2\exp {-\frac {a}{2}l} \max \set { \sqrt {\frac {q}{2\pi }},\, q,\, avq^{3/2}\sqrt {\frac {\pi }{2}}} \left (1+2\exp {-\frac {l^2}{8v^2q}}\right )\\ &\leq && C_1J^2\max \set {q^{1/2},\,q^{3/2}}\exp {-c_1l}, \end {alignat*} with $C_1$ and $c_1$ defined in an obvious way as above. This completes the proof.\end{proof}
\label{proofsection:prAtEndv}\begin{proof}[Proof of \autoref{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Recall from Lemma \ref {lemma:ml} that we applied Lieb-Robinson to operators such as $\i \comm {H}{H_L}(\tau )$. By Assumption \ref {ass:op}, since $H$ and $H_L$ are self-adjoint, the commutators are bounded and one has $\adj {\i \comm {H}{H_L}}=-\i \left (H_LH-HH_L\right )=\i \comm {H}{H_L}$ $\Rightarrow $ we can conclude that the commutator is self-adjoint. Applying Lieb-Robinson as in \cite [Lemma 3.2]{NearComm}, one can construct the local approximation to preserve self-adjointness. We briefly elaborate. \par Let $\X =\X _1\otimes \X _2$. For the construction of $\Pi :\LL {\X }\rightarrow \LL {\X }$ in \cite [Lemma 3.2]{NearComm}, the authors use an arbitrary state\footnote {Positive operator with unit trace norm.} $\rho :\X _2\rightarrow \X _2$, though the resulting bound does not depend on the choice of $\rho $. Then, for this state, applying the spectral decomposition, we have \begin {align*} \rho =\sum _{k=1}^\infty \lambda _k\inp {\cdot }{\bs \psi _k}_{\X _2}\bs \psi _k, \end {align*} for $\set {\bs \psi _k:\;k\in \N }$ orthonormal in $\X _2$. Next, for each $\bs \psi _k$, the authors define the map $A_k$ as \begin {align*} \inp {\bs v}{A_k\bs w}_{\X _1}=\inp {\bs v\otimes \bs \psi _k}{A\bs w\otimes \bs \psi _k}_{\X },\quad \forall \bs v,\,\bs w\in \X _1. \end {align*} Finally, the map $\Pi (A)$ is defined as \begin {align*} \Pi (A):=\left (\sum _{k=1}^\infty \lambda _kA_k \right )\otimes \id . \end {align*} Note that each $A_k$ is self-adjoint if $A$ is self-adjoint. Therefore, $\Pi (A)$ is self-adjoint. \par Thus, $M_L$, $M_B$ and $M_R$ can be chosen self-adjoint. By Lemmas \ref {lemma:ml} and \ref {lemma:ann}, picking $q=c_1\frac {2l}{(\Delta E)^2}$, we get $\norm {M_L\uu _0}[\X ]\leq C_1J^2\max \set {q^{1/2},\,q^{3/2}}\exp {-c_1l}$. Moreover, since $M_L$ is self-adjoint, there exists a projection valued measure $P(\cdot )$ such that \begin {align*} \normsq {M_L\uu _0}{\X }=\inp {M_L\uu _0}{M_L\uu _0}_{\X }= \inp {\uu _0}{M_L^2\uu _0}_{\X }=\int _{\sigma (M_L)}\lambda ^2\d P_{\uu _0}(\lambda ). \end {align*} \par We split the spectrum of $M_L$ as \begin {align*} \sigma _1(M_L)&:=\set {\lambda \in \sigma (M_L):|\lambda |\leq C_1J^2\max \set {q^{1/2},\,q^{3/2}}\exp {-c_1l/2}},\\ \sigma _2(M_L)&:=\sigma (M_L)\setminus \sigma _1(M_L). \end {align*} Define $L$ as \begin {align*} L:=\int _{\sigma _1(M_L)}\d P(\lambda ). \end {align*} Clearly, $L$ is a bounded self-adjoint operator with $\norm {L}[\Lnorm ]=1$ and the same support as $M_L$. Moreover, by orthogonality of the spectral subspaces \begin {align*} C_1^2J^4\max \set {q,\,q^{3}}\exp {-c_12l}&\geq \norm {M_L\uu _0}[\X ] = \int _{\sigma _1(M_L)}\lambda ^2\d P_{\uu _0}(\lambda )\uu _0+ \int _{\sigma _2(M_L)}\lambda ^2\d P_{\uu _0}(\lambda )\uu _0\\ &\geq C_1^2 J^4\max \set {q,\,q^{3}} \exp {-c_1l}\int _{\sigma _2(M_L)}\d P_{\uu _0}(\lambda ). \end {align*} Thus, $\int _{\sigma _2(M_L)}\d P_{\uu _0}(\lambda )\leq \exp {-c_1l}$. Finally, this gives \begin {align*} \norm {(L-\id )\uu _0}[\X ]&= \norm {\int _{\sigma _2(M_L)}\d P(\lambda )\uu _0}[\X ]= \left (\int _{\sigma _2(M_L)}\d P_{\uu _0}(\lambda )\right )^{1/2}\\ &\leq \exp {-c_1l/2}. \end {align*} Analogously for $R$. This completes the proof.\end{proof}
\label{proofsection:prAtEndvi}\begin{proof}[Proof of \autoref{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Note that $H=\tilde {H}_L+\tilde {H}_B+ \tilde {H}_R$. By utilizing the estimates from Lemma \ref {lemma:ml}, we have \begin {align}\label {eq:exp} &\norm {\frac {1}{N\sqrt {2\pi q}}\int _{-\infty }^\infty \big \{\exp {\i (\tilde {H}_L+\tilde {H}_B+\tilde {H}_R )t}\notag -\exp {\i (M_L+M_B+M_R)t}\big \}\exp {-\frac {t^2}{2q}}\d t}[\Lnorm ]\notag \\ &\leq 3C_1(1/N)J^2\max \set {q^{1/2},\, q^{3/2}}\exp {-c_1l} \frac {1}{\sqrt {2\pi q}}\int _{-\infty }^\infty |t| \exp {-\frac {t^2}{2q}}\d t\\ &=3(2\pi )^{-1/2}C_1(1/N)J^2 \max \set {q,\, q^{2}}\exp {-c_1l}\notag , \end {align} where the inequality can be shown using \cite [Chapter 9, Theorem 2.12, Equation (2.22)]{Kato}. \par Next, for the exponential term we can write \begin {align*} &\exp {\i (M_L+M_B+M_R)t} =\exp {\i (M_L+M_B+M_R)t}\exp {-\i (M_L+M_R)t} \exp {\i (M_L+M_R)t}, \end {align*} and we define $U(t):=\exp {\i (M_L+M_B+M_R)t}\exp {-\i (M_L+M_R)t}$. In $U(t)$ the term in the exponent commutes for different $t$, since the time-dependence is a simple multiplication by $t$. We thus compute \begin {align*} &\frac {\d }{\d t}U(t) =\exp {\i (M_L+M_B+M_R)t}\i (M_L+M_B+M_R) \exp {-\i (M_L+M_R)t}\\ &- \exp {\i (M_L+M_B+M_R)t}\i (M_L+M_R) \exp {-\i (M_L+M_R)t}\\ &=\exp {\i (M_L+M_B+M_R)t}\i M_B\exp {-\i (M_L+M_R)t}\\ &=\exp {\i (M_L+M_B+M_R)t}\exp {-\i (M_L+M_R)t} \exp {\i (M_L+M_R)t}\i M_B\exp {-\i (M_L+M_R)t}\\ &=U(t)\exp {\i (M_L+M_R)t}\i M_B\exp {-\i (M_L+M_R)t} \end {align*} and $U(0)=\id $. We abbreviate \begin {align*} M_B(t):=\exp {\i (M_L+M_R)t}M_B\exp {-\i (M_L+M_R)t}. \end {align*} Due to the simple form of $\i M_B(t)$, the solution to this initial value problem exists, is unique and is given by the (negative) time-ordered exponential of $\i M_B(t)$, see \cite [Chapter X.12]{MathPhys2} (interaction representation) or \cite {Unbounded} for ordered exponentials of more general unbounded time-dependent Hamiltonians. \par Thus, our approximation so far is \begin {align*} \bar {\rho }^q=\frac {1}{N\sqrt {2\pi q}}\int _{-\infty }^\infty \adj {\oe {A}{0}{t}}\exp {\i (M_L+M_R)t}\exp {-\frac {t^2}{2q}}\d t. \end {align*} By multiplying $L$, $R$ from the right we obtain \begin {align*} &\norm {\bar {\rho }^qLR-P_0}[\Lnorm ] =\norm {(\bar {\rho }^q-P_0+P_0)LR-P_0}[\Lnorm ] =\norm {(\bar {\rho }^q-P_0)LR+P_0LR-P_0}[\Lnorm ] \\ &\leq \norm {\bar {\rho }^q-P_0}[\Lnorm ]+ \norm {P_0LR-P_0}[\Lnorm ]. \end {align*} For the latter term we use Lemma \ref {lemma:ol}, set $q=c_1\frac {2l}{(\Delta E)^2}$ and obtain \begin {align*} &\norm {P_0LR-P_0}[\Lnorm ]= \norm {P_0 \left \{(L-\id +\id )+(R-\id +\id )-\id \right \} }[\Lnorm ]\\ &=\norm {P_0(L-\id )(R-\id )+P_0(L-\id )+ P_0(R-\id ) }[\Lnorm ]\\ &\leq 3\norm {(L-\id )P_0}[\Lnorm ]+ \norm {(R-\id )P_0}[\Lnorm ] \leq 4\exp {-c_1l/2}. \end {align*} since $\norm {P_0}[\Lnorm ]= \norm {L}[\Lnorm ]=1$ and $P_0$, $L$ and $R$ are self-adjoint. Thus, overall \begin {align*} \norm {\bar {\rho }^qLR-P_0}[\Lnorm ]&\leq 3(2\pi )^{-1/2}(1/N)C_1J^2\max \set {q,\, q^2}\exp {-c_1l} +4\exp {-c_1l/2}. \end {align*} \par Finally, by definition, $L$ and $R$ project onto the spectral subspaces of $M_L$ and $M_R$ corresponding to small eigenvalues. I.e., \begin {align*} \norm {\left [\exp {\i (M_L+M_R)t}-\id \right ]LR }[\Lnorm ]\leq 2|t|C_1J^2\max \set {q^{1/2},\,q^{3/2}} \exp {-c_1l/2}, \end {align*} \par hence \begin {align*} \norm {\bar {\rho }^qLR-\tilde {\rho }^q}[\Lnorm ] &\leq \bigg \|\frac {1}{N\sqrt {2\pi q}}\int _{-\infty }^\infty \adj {\oe {A}{0}{t}}\times \\ &\exp {-\frac {t^2}{2q}}\left (\exp {\i (M_L+M_R)t}LR-LR \right )\d t\bigg \|_{\Lnorm }\\ &\leq 2C_1(1/N)J^2\max \set {q^{1/2},\, q^{3/2}}\exp {-c_1l/2} \frac {1}{\sqrt {2\pi q}}\int _{-\infty }^\infty |t|\exp {-\frac {t^2}{2q}}\d t\\ &= C_1(1/N)J^2(2\pi )^{-1/2}\max \set {q,\,q^2}\exp {-c_1l/2}. \end {align*} \par Overall we obtain \begin {align*} \norm {\tilde {\rho }^q-P_0}[\Lnorm ]&\leq \norm {\bar {\rho }^qLR-P_0}[\Lnorm ]+ \norm {\bar {\rho }^qLR-\tilde {\rho }^q}[\Lnorm ]\\ &\leq C_2J^2\max \set {q,\, q^2}\left ( \exp {-c_1l/2}+\exp {-c_1l}\right ), \end {align*} for an appropriately chosen constant $C_2>0$. This completes the proof.\end{proof}
\label{proofsection:prAtEndvii}\begin{proof}[Proof of \autoref{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}We use the same technique as in Lemma \ref {lemma:ml} to show that the non-local part of $M_B(t)$ is bounded. \begin {align*} M_B(t)&:=\exp {\i (M_L+M_R)t}M_B\exp {\i (M_L+M_R)t},\\ \frac {\d }{\d t}M_B(t)&=\exp {\i (M_L+M_R)t}\comm {M_L+M_R}{M_B} \exp {-\i (M_L+M_R)t},\\ \comm {M_L+M_R}{M_B}&=\comm {H_L}{H_B}+\comm {H_L}{\diff _B}+ \comm {\diff _L}{H_B}+\comm {\diff _L}{\diff _B}+ \comm {H_R}{H_B}\\ &+\comm {H_R}{\diff _B}+\comm {\diff _R}{H_B} +\comm {\diff _R}{\diff _B}. \end {align*} Since $\diff _L$ and $\diff _R$ are supported on a superset of the supports of $\comm {H}{H_L}$ and $\comm {H}{H_R}$, we obtain \begin {align*} \supp {\comm {M_L+M_R}{M_B}} \subset \supp {\diff _L}\cup \supp {\diff _R}=\supp {M_B}. \end {align*} Thus, as in Lemma \ref {lemma:ml}, we can approximate $M_B(t)$ by a local operator $\tilde {M}_B(t)$ supported on $\X _{j-3l-2,j+3l+3}$ such that \begin {align*} \norm {M_B(t)-\tilde {M}_B(t)}[\Lnorm ]\leq CJ^2|t|\exp {-a\{l-v|t|\}}. \end {align*} We utilize this estimate in a similar way as in \eqref {eq:exp}. To this end, we write the time-ordered exponential as a product integral and use a step function approximation to the integral (see \cite [Chapter 3.6]{ProductInt}), namely \begin {align*} \adj {\oe {A}{0}{t}}=\prod _{0}^t\exp {A(\tau )}\d \tau = \lim _{K\rightarrow \infty }\left ( \exp {A(t_K)\Delta t}\cdots \exp {A(t_0)\Delta t}\right ), \end {align*} where $t_i=i\Delta t$, $\Delta t=t/K$ and the convergence is meant in the strong sense. This is possible due to the simple form of $A(t)$, i.e., $\exp {A(t)}$ is bounded with norm 1. \par For $K=1$, we obtain as in \eqref {eq:exp} \begin {align*} \norm {\exp {\i M_B(t)\Delta t}-\exp {\i \tilde {M}_B(t)\Delta t} }[\Lnorm ]\leq |\Delta t|\norm {M_B(t)-\tilde {M}_B(t) }[\Lnorm ], \end {align*} with $|\Delta t|=|t|$. For $K-1\rightarrow K$, by induction \begin {align*} &\norm {\exp {\i M_B(t_K)\Delta t}\cdots \exp {\i M_B(t_0)\Delta t}- \exp {\i \tilde {M}_B(t_K)\Delta t}\cdots \exp {\i \tilde {M}_B(t_0)\Delta t} }[\Lnorm ]\\ &\leq \norm {\left [\exp {\i M_B(t_K)\Delta t}- \exp {\i \tilde {M}_B(t_K)\Delta t}\right ] \exp {\i M_Bt_{K-1}\Delta t} \cdots \exp {\i M_B(t_0)\Delta t}}[\Lnorm ]\\ &+ \bigg \|\exp {\i \tilde {M}_B(t_K)\Delta t} \times \\ &\left [\exp {\i M_B(t_{K-1})\Delta t}\cdots \exp {\i M_B(t_0)\Delta t}- \exp {\i \tilde {M}_B(t_{K-1}) \Delta t}\cdots \exp {\i \tilde {M}_B(t_0)\Delta t}\right ]\bigg \|_{\Lnorm }\\ &\leq |\Delta t|K \norm {M_B(t)-\tilde {M}_B(t)}[\Lnorm ], \end {align*} where by definition $|\Delta t|K=|t|$. Thus, we can estimate for the ordered exponential \begin {align*} &\norm {\adj {\oe {\i M_B}{0}{t}}-\adj {\oe {\i \tilde {M}_B}{0}{t}}}[\Lnorm ]\\ &\leq |t|\norm {M_B(t)-\tilde {M}_B(t)}[\Lnorm ] \leq CJ^2t^2\exp {-a\{l/3-v|t|\}}. \end {align*} We define the local operator $B$ as \begin {align*} B:=\frac {1}{N\sqrt {2\pi q}}\int _{-\infty }^\infty \adj {\oe {\i \tilde {M}_B}{0}{t}}\exp {-\frac {t^2}{2q}}\d t. \end {align*} Estimating as in \eqref {eq:trunc} for $T=\frac {l}{6v}$, we obtain \begin {align*} &\norm {\OB -B}[\Lnorm ]\leq \norm {\int _{|t|\leq T\ldots }+\int _{|t|>T}\ldots }[\Lnorm ] \leq C(1/N)J^2\exp {-al/3}\\ &\times \left (\exp {avT}\frac {1}{\sqrt {2\pi q}}\int _{|t|\leq T} t^2\exp {-\frac {t^2}{2q}}\d t+ \frac {1}{\sqrt {2\pi q}}\int _{|t|>T}t^2\exp {av|t|-\frac {t^2}{2q}}\d t \right ). \end {align*} In analogy to \eqref {eq:trunc}, for the first term we obtain \begin {align*} \frac {1}{\sqrt {2\pi q}}\int _{|t|\leq T} t^2\exp {-\frac {t^2}{2q}}\d t\leq \frac {q}{2}. \end {align*} For the second term, applying integration by parts, we obtain \begin {align*} &\frac {1}{\sqrt {2\pi q}}\int _{|t|>T}t^2\exp {av|t|-\frac {t^2}{2q}}\d t= \sqrt {\frac {2}{\pi q}}\int _{T}^\infty t^2\exp {avt-\frac {t^2}{2q}}\d t\\ &=\sqrt {\frac {2}{\pi q}}\bigg ( Tq\exp {avT-\frac {T^2}{2q}}+q\int _{T}^\infty \exp {avt-\frac {t^2}{2q}} dt +avq\int _{T}^\infty t\exp {avt-\frac {t^2}{2q}}\d t\bigg ). \end {align*} And hence \begin {align*} &\frac {1}{\sqrt {2\pi q}}\int _{|t|>T}t^2\exp {av|t|-\frac {t^2}{2q}}\d t \leq \exp {avt-\frac {T^2}{2q}}\frac {\sqrt {2}}{\sqrt {\pi }|1-avq|} \sqrt {q}\left (\sqrt {\frac {q\pi }{2}+T}\right ). \end {align*} The final estimate is thus \begin {align*} \norm {\OB -B}[\Lnorm ]\leq C_3J^2\max \set {q^{1/2},\, q}\exp {-3c_3l}, \end {align*} for appropriate constants $C_3>0$, $c_3>0$. This completes the proof.\end{proof}

